Distribution-Aware Sampling and Weighted Model Counting for SAT

Given a CNF formula and a weight for each assignment of values to variables, two natural problems are weighted model counting and distribution-aware sampling of satisfying assignments. Both problems have a wide variety of important applications. Due to the inherent complexity of the exact versions of the problems, interest has focused on solving them approximately. Prior work in this area scaled only to small problems in practice, or failed to provide strong theoretical guarantees, or employed a computationally-expensive maximum a posteriori probability (MAP) oracle that assumes prior knowledge of a factored representation of the weight distribution. We present a novel approach that works with a black-box oracle for weights of assignments and requires only an {\NP}-oracle (in practice, a SAT-solver) to solve both the counting and sampling problems. Our approach works under mild assumptions on the distribution of weights of satisfying assignments, provides strong theoretical guarantees, and scales to problems involving several thousand variables. We also show that the assumptions can be significantly relaxed while improving computational efficiency if a factored representation of the weights is known.

==> Introduction-SC.tex <==
\section{Introduction}
Given a set of weighted elements and a constraint over them, finding
the cumulative weight of all elements that satisfy the constraint is a
fundamental problem that arises in many contexts.  Known variously as
weighted model counting, discrete integration and partition function
computation, this problem has applications in machine learning,
probabilistic reasoning, statistics, planning and combinatorics, among
other areas~\cite{}.  A closely related problem is that of sampling
elements satisfying a constraint, where the probability of sampling an
element is proportional to its weight.  The latter problem, known as
weighted sampling, also has important applications in probabilistic
reasoning, machine learning, statistical physics, constrained random
verification and other domains~\cite{jerrum-sinclair,madras,others}.
Unfortunately, the exact versions of both problems are computationally
hard.  Weighted model counting can be used to count the number of
satisfying assignments of a CNF formula; hence it is
$\#P$-hard~\cite{valiant79}.  %
%
%
It is known that an efficient algorithm for weighted sampling would
yield a fully polynomial randomized approximation scheme (FPRAS) for
{\#P}-complete inference problems~\cite{jerrum-sinclair,madras} -- a
possibility for which we do not yet have any evidence.  Fortunately,
approximate solutions to the weighted model counting and weighted
sampling problems are good enough for most applications.  Hence, there
has been considerable interest in designing practical algorithms for
these approximate problems.

In their seminal paper~\cite{JVV}, Jerrum, Valiant and Vazirani showed
that approximate model counting and almost uniform sampling (a special
case of approximate weighted sampling) are polynomially
inter-reducible.  Therefore, hardness of one problem implies hardness
of the other.  Roth showed that approximating the count of satisfying
assignments of a CNF formula is {\NP}-hard, even with severe
restrictions on the sizes of clauses and occurrences of
variables~\cite{Roth1996}.  Therefore, polynomial-time algorithms for
approximate weighted model counting or approximate weighted sampling
are highly unlikely.  Recently, a new class of algorithms that use
pairwise independent random parity constraints and a {\MAP}
\emph{(maximum a posteriori probability)}-oracle have been proposed
for approximately solving the weighted model counting and weighted
sampling problems~\cite{ermon2013icml,ermon2014icml,ermon2013nips}.
These algorithms provide strong theoretical guarantees (FPRAS relative
to the oracle), and have been shown to scale to medium-sized problems
in practice.  While this represents a significant step forward in our
quest for practically efficient algorithms with strong theoretical
guarantees for approximate weighted model counting and approximate
weighted sampling, the simultaneous use of {\MAP}-queries and parity
constraints raises questions about the scalability of the proposed
algorithms to larger problem instances~\cite{ermon2013uai}.
Interestingly, random parity constraints and a SAT solver
({\NP}-oracle) engineered to analyze parity constraints efficiently
has been used in earlier work~\cite{CSM-cav13,CSM-cp13,MeelMSThesis14}
to design highly scalable algorithms for approximate model counting
and almost uniform sampling in the unweighted case.  In this paper, we
argue that it is possible to extend the same paradigm and avoid calls
to an expensive {\MAP} solver completely to solve the corresponding
problems in the weighted case, under mild assumptions about the
distribution of weights.



%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

In a large class of problems arising in practice, we observed that
given a set of constraints, the ratio {\ratio} of the maximum weight of
a satisfying assignment to the minimum weight of a satisfying
assignment, can be conservatively bounded above by not-so-large
numbers.  We exploit this property crucially in evading MAP queries in
our work.  Significantly, this also allows us to break free from the
requirement that weights of assignments must be given in a form
(viz. graphical probabilistic models) that allow efficient MAP
inferencing.  Indeed, our algorithms makes no assumptions on the way
in which weights of assignments are computed, and work with a
black-box model for computing weights.  We show that if {\ratio} is
small enough (say $< 5$), random partitioning-based algorithms for
approximate (unweighted) model counting and almost uniform generation,
presented earlier in~\cite{SKV13MC,SKV13}, can be adapted to perform
approximate weighted model counting and approximate distribution-aware
generation.  Like the original algorithms in~\cite{SKV13MC,SKV13}, the
adapted algorithms only assume access to a SAT solver that accepts a
CNF formula and a set of parity constraints as inputs.  We show
further that if $\log \ratio$ is small (say $< 10$), the adapted
algorithms obtained above can themselves be used as subroutines in
newer algorithms that solve the approximate weighted model counting
and approximate distribution-aware generation problems.  However,
these newer algorithms assume access to a pseudo-Boolean solver that
accepts a CNF formula, a set of parity constraints and linear
inequality constraints as inputs.  All algorithms presented in this
paper compute results that are provably within a specified tolerance
$\varepsilon$ with high probability.  Performance-wise, experimental
results confirm (hopefully ?)  that using a propositional SAT solver,
or a pseudo-Boolean solver, is more efficient and less restrictive in
practice than using a MAP query solver.  This vindicates our approach
and opens up possibilities of further research on MAP query-free
algorithms that use propositional or pseudo-Boolean solvers as
oracles.

The remainder of the paper is organized as follows.

